Explicit mathematical epidemiology results on age renewal kernels and R0 formulas are often consequences of the rank one property of the next generation matrix

A very large class of ODE epidemic models (2.2) discussed in this paper enjoys the property of admitting also an integral renewal formulation, with respect to an "age of infection kernel" a(t) which has a matrix exponential form (3.2). We observe first that a very short proof of this fact is available when there is only one susceptible compartment, and when its associated "new infections" matrix has rank one. In this case, a(t) normalized to have integral 1, is precisely the probabilistic law which governs the time spent in all the "infectious states associated to the susceptible compartment", and the normalization is precisely the basic replacement number. The Laplace transform (LT) of a(t) is a generalization of the basic replacement number, and its structure reflects the laws of the times spent in each infectious state. Subsequently, we show that these facts admit extensions to processes with several susceptible classes, provided that all of them have a new infections matrix of rank one. These results reveal that the ODE epidemic models highlighted below have also interesting probabilistic properties.

==> cts.tex <==
\ssec{The importance of  computational aspects in the study of dynamical systems}
It may be argued that nowadays, all papers written on    applied dynamic models should be  approached from a computational science point of view.
Indeed, the fundamental  problems of determining the  number of fixed points and limit cycles,  and of  identifying  bifurcations (Hopf, saddle-node, Bogdanov-Takens), etc,  reduce all to the solution of polynomial systems of  equalities or inequalities. Now  the modern tools  for  tackling symbolically such problems come  from algebraic geometry (like Groebner bases).

Sometimes, CAS's (which use Groebner bases for solving) solve our problems   immediately, sometimes one needs to   ``twist"  the  notebook before reaching a result, and  sometimes one needs to plug in a numeric condition (possibly with parameters  determined by physical experimentation).
In all these cases, the notebook becomes a crucial part of a paper.

The remarkable  opportunity we have nowadays of being able to accompany our pencil calculations with electronic notebooks was emphasized already 30 years ago in  papers like
``Electronic documents give reproducible research a new meaning" \cite{Repro} -- see also \cite{buckheit1995wavelab,Donoho}. Following the efforts of numerous people,  lots of progress has been achieved in this direction, as witnessed in particular by the existence of the platform GitHub.

\subsection{ A critic of the mathematical epidemiology bifurcations literature}

 We believe that a great part of the mathematical epidemiology literature  suffers today from two   draw-backs.
\BEN \im   The major one  is the lack of ``electronic reproducibility", i.e.  of  notebooks made public.
Here, we provide  electronic notebooks   for the papers cited above,  where the reader may  recover the results,  and also modify  them as he pleases, for analyzing similar models.
We believe that electronic  reproducibility in the above sense  should    be  the norm in the  field of mathematical biology.

 \im A  second draw-back in our opinion is the focus on particular cases, furthermore studied under simplifying assumptions, which are  often  difficult to justify epidemiologically, like assuming $0$ deaths or eternal immunity. It seems sometimes  that  the   justification of the simplifying assumptions is to  allow a ``solution by hand", in the spirit of ``mathematics olympiad problems". Solving particular cases may of course be quite useful pedagogically, but is not efficient.  For just one of many examples where symbolic computing beats easily hand computations,
 note that the ``mathematics olympiad literature" restricts itself often to polynomials  of order $2$, to be able to use their elementary discriminant formula, which is of course unnecessary nowadays. 
 We believe that mathematical epidemiology
 could be better served by relying more heavily on  modern symbolic computation. As another benefit,  from this point of view  there is no need  to dedicate separate papers  to each  particular case  of general models like \eqr{Vys}.  A more natural approach   would be to study unified general cases symbolically as far as possible (until encountering time constraints),   pinpointing  how far can one push symbolics, and  turn to symbolic or  numeric particular cases only subsequently.
 
 Below, we investigate our model at two levels:
 \BEN \im The general one in \eqr{ZFG}, for which we may already provide simple information, like $R_0$, and the maximum possible number of fixed points.
 \im The particular case \eqr{ZF}, for which we are able to provide bifurcation results  as well.

 We believe that the traditional paradigm of one model, one paper doesn't suit well  mathematical epidemiology, where the interesting model for epidemiologists is always quite  general, but mathematicians  are only able to solve completely  just particular cases (which may be uninteresting  for epidemiologists).
\EEN


\EEN

{\bf Contributions}. Our motivation for   revisiting the bifurcation work of  \cite{ZhouFan}  was   the desire to accomplish the  task of
{ providing an electronic notebook, which may eventually be easily modified for studying variations of similar models}.
This quite non-trivial task required in particular pinpointing the ``symbolic-numeric boundary" for this problem, which turned out to be the computation of the trace at the stable endemic point $E_2$. This calculation was first achieved in numeric instances, but finally also symbolically by Mathematica, and lead to the introduction of some interesting symbolic objects, ''Groebner eliminated traces and determinants" -- see \eqr{dt}, \eqr{Gdt}, which seem  to have appeared here for the first time.

 



{\bf Contents}.
Our paper starts in section \ref{s:his} highlights of  previous  literature concerning the SIRS model with nonlinear force of infection and treatment. 
It then formulates in section \ref{s:ZFG}, \eqr{ZFG}, a general epidemic model, for which $R_0$ and the ``scalarization" of the fixed point system are easily achieved. The analysis of the simplest particular case  $ \g_r=\g_s=i_s=0$, studied in \cite{ZhouFan,Gupta}, is then revisited and corrected in Section \ref{s:ZF}.  
Section \ref{s:Gro} introduces the interesting  ''Groebner eliminated traces and determinants"  \eqr{dt}, \eqr{Gdt}, which turn out useful in the determination of Bogdanov-Takens bifurcations. Sections \ref{s:Fanb}, \ref{s:tpp} complete  aspects missing in the original papers concerning the two-parameter bifurcation diagram and the  important ``corners where several regions meet".
Last but not least, our  paper is accompanied   by electronic notebooks supporting the results.
%Finally, we  structure our work in a way that will lay out the foundations   in the future treating the \cite{Perez} model, the unification \eqr{ZFP}, as well as the three dimensional model \eqr{Vys}.



%Section \ref{s:app} provides further details on the computation of the endemic points.

\iffalse
 and section \ref{s:num} provides further details on our symbolic and numeric notebooks.

 General results which hold without treatment, under the umbrella of \eqr{Vys},   are presented in
Section \ref{s:prel}.  We turn then

We include last, for completeness,   a  review of the Poincar\'e-Andronov-Hopf and Bermuda triangle bifurcations in Section \ref{s:Hop}.
\fi

